Distributed, partially collapsed MCMC for Bayesian Nonparametrics

Bayesian nonparametric (BNP) models provide elegant methods for discovering underlying latent features within a data set, but inference in such models can be slow. We exploit the fact that completely random measures, which commonly used models like the Dirichlet process and the beta-Bernoulli process can be expressed as, are decomposable into independent sub-measures. We use this decomposition to partition the latent measure into a finite measure containing only instantiated components, and an infinite measure containing all other components. We then select different inference algorithms for the two components: uncollapsed samplers mix well on the finite measure, while collapsed samplers mix well on the infinite, sparsely occupied tail. The resulting hybrid algorithm can be applied to a wide class of models, and can be easily distributed to allow scalable inference without sacrificing asymptotic convergence guarantees.

==> old_background.tex.tex <==
%\section{Background and Related Work}\label{sec:bnp}
\section{Background and Related Work}\label{sec:bnp}
%\subsection{Bayesian nonparametric priors derived from completely random measures}

%\sinead{For AISTATS let's cut down the background, inference approaches, and distributed inference methods, sections to less than a page.}

Completely random measures (CRMs) \citep{Kingman:1967} are random measures $\mu$ on some space $\Omega$, where the masses $\mu(A_i), \mu(A_j)$ assigned to disjoint subsets $A_i, A_j\subset \Omega$  are independent. For example, the gamma process with base measure $M$ assigns a $\mbox{Gamma}(M(A))$ mass to any subset $A\subset \Omega$. Other examples include the beta process \citep{Hjort:1990} and the Poisson process.

Many commonly used exchangeable nonparametric distributions can be expressed in terms of CRMs. For example, if we sample $B = \sum_{i=1}^\infty \mu_i \delta_{\theta_i}$ from a (homogeneous) beta process, and generate a sequence of subsets $Z_i$ where $\theta_k\in Z_i$ w.p.\ $\mu_k$, then the marginal distribution over the $Z_i$ is described (up to a reordering) by the Indian buffet process. If we sample $G= \sum_{i=1}^\infty \gamma_i \delta_{\theta_i}$ from a gamma process with base measure $\alpha H$, then $D= \sum_{i=1}^\infty \pi_i \delta_{\theta_i}$, where $\pi_i = \gamma_i/\sum_j\gamma_j$ is distributed according to a Dirichlet process with concentration parameter $\alpha$ and base measure $H$. If we then generate a sequence of cluster indicators $Y_i$ where $Y_i=k$ w.p.\ $\pi_k$, then the resulting partition is described (up to a reordering) by the Chinese restaurant process.

%Inference in the resulting exchangeable distributions tends to fall into two categories: uncollapsed methods that (partially, or approximately) instantiate the latent CRM or normalized CRM and alternate between sampling the latent measure and the assignments \citep{Ishwaran:Zarepour:2002,Paisley:Carin:2009,Zhou:2009,Walker:2007,Ge:Chen:Wan:Ghahramani:2015,Teh:Gorur:Ghahramani:2007}, and collapsed methods where the latent measure is integrated out \citep{Ishwaran:James:2001,Neal:1998,Griffiths:Ghahramani:2005}. 

\iffalse
We can create probability measures by normalizing CRMs: for example, a Dirichlet process with concentration parameter $\alpha$ and base measure $H$ corresponds to the normalization of a gamma process with base measure$\alpha H$. We can also create exchangeable distributions by using a CRM as a mixing measure: for example, if we sample $B = \sum_{i=1}^\infty \mu_i \delta_{\theta_i}$ from a (homogeneous) beta process, and generate a sequence of subsets $Z_i$ where $\theta_k\in Z_i$ w.p.\ $\mu_k$, then the marginal distribution over the $Z_i$ is described (up to a reordering) by the Indian buffet process.

Inference in nonparametric models based on CRMs typically follows tw





Many commonly used nonparametric priors, including the Dirichlet process and the Indian buffet process, can be expressed in terms of a class of distributions known as completely random measures (CRM) \citep{Kingman:1967}. A completely random measure is a random measure $\mu$ on some space $\Omega$ where the masses $\mu(A_i), \mu(A_j)$ assigned to disjoint subsets $A_i, A_j\subset \Omega$  are independent.


A commonly used example of a completely random measure is the gamma process. If $H$ is some probability measure on $\Omega$, and $\alpha>0$, then the gamma process assigns a $\mbox{Gamma}(\alpha H(A))$ mass to any subset $A\subset \Omega$. 
The Dirichlet process is a distribution over random probability measure $D\sim \mbox{DP}(\alpha, H)$ on $\Omega$ that corresponds to the normalization of a gamma process with parameters $\alpha$ and $H$. Since the gamma process assigns independent gamma-distributed masses to disjoint subsets of $\Omega$, the masses assigned by a Dirichlet process to a finite partition of $\Omega$ are necessarily Dirichlet distributed, i.e. if $A_1,\dots,A_K$ is a partition of $\Omega$, then $(D(A_1),\dots, D(A_k)) \sim \mbox{Dirichlet}(\alpha H(A_1), \dots, \alpha H(A_K))$.

We can use a Dirichlet process-distributed random measure 
\begin{equation}
D:=\sum_{k=1}^\infty \pi_k \delta_{\theta_k}
\end{equation}
to assign parameters to observations:
\begin{equation}
  \begin{split}
    D\sim& \mbox{DP}(\alpha, H)\\
    \phi_n \sim& D
  \end{split}
\end{equation}
The discrete nature of $D$ means that a single atom $\pi_k\delta_{\theta_k}$ can be associated with multiple observations, so we will get repeated values of $\phi_n$, so that we are partitioning observations into an unbounded number of clusters. If we let $z_n$ be the cluster indicator for the $n$th data point, we can directly obtain the predictive distribution over $z_{n+1}|z_{1:n}$:

\begin{equation}
  P(z_{n+1} = k|z_{1:n}, \alpha) = \begin{cases} \frac{m_k}{n+\alpha} & \mbox{for } k\leq K\\
    \frac{\alpha}{n+\alpha} & \mbox{for }k=K+1
  \end{cases}\label{eqn:crp}
\end{equation}
where $K$ is the number of clusters present in the first $n$ observations, and $m_k$ is the number of observations in the $k$th cluster. To recover a full mixture model from Equation~\ref{eqn:crp}, we can sample a cluster parameter $\theta_k \sim H$ for each cluster and set $\phi_n:=\theta_{z_n}$.

Another commonly used CRM is the beta process \citep{Hjort:1990,Thibaux:Jordan:2007}. The (homogenous) beta process is a completely random measure where the distribution over atom sizes is given by the limit, as $K\rightarrow \infty$, of a $\mbox{Beta}\left(c\frac{\alpha}{K},c\left(1-\frac{\alpha}{K}\right)\right)$ distribution, and whose atom locations are i.i.d. according to some probability measure $H$. The beta process can be used as a prior for latent feature models. If $B:=\sum_{k=1}^\infty \mu_k \delta_{\theta_k}\sim \mbox{BP}(\alpha, c, H)$, then we can interpret the $\mu_k$ as the probability of an observation containing the $k$th latent feature $\theta_k$. We can select a finite subset of these latent features for the $n$th data point by sampling a sequence $Z_n$ of binary indicator variables $z_{n,k}\sim\mbox{Bernoulli}(\mu_k)$.

As with the Dirichlet process, it is possible to integrate out the latent measure and work directly with the predictive distribution over the binary sequences. If $K$ is the number of features seen in the first $n-1$ data points, then we can sample the next sequence $Z_{n}=(z_{n,k})_{k=1}^\infty$ as
\begin{equation}
  \begin{split}
    z_{n,k} &\sim \mbox{Bernoulli}\left(\frac{m_k}{n}\right), \qquad  k=1,\dots,K\\
    J &\sim \mbox{Poisson}\left(\frac{\alpha}{n}\right)\\
    z_{n,j} &= 1, \qquad j=K+1, \dots, K+J\\
    z_{n,j} &= 0, \qquad j>K+J\\
    K\leftarrow& K+J
  \end{split}\label{eqn:ibp}
\end{equation}
If we stack the sequences $Z_n$ into a matrix $\mathbf{Z}$, Equation~\ref{eqn:ibp} describes a distribution over binary matrices known as the Indian buffet process \citep{Griffiths:Ghahramani:2005}.

%\subsection{Inference approaches}\label{sec:existing_inf}
\section{Inference approaches}\label{sec:existing_inf}
In Section~\ref{sec:bnp}, we saw two complementary representations for the cluster/latent variable allocations obtained using a Dirichlet process and an Indian buffet process. We can either explicitly instantiate the latent measure and sample each data point's allocations independently given this measure, or we can integrate out the latent measure and work directly with the predictive distribution.

When designing an MCMC algorithm, these two options lead directly to two different inference approaches, which we will refer to as \textit{collapsed} and \textit{uncollapsed} samplers. In an uncollapsed sampler, we alternate between sampling the random measure given the cluster/latent feature allocations, and sampling the allocations given the random measure. To avoid having to instantiate the infinitely many atoms of the random measure, we can either replace the random measure with a finite-dimensional approximation (see \cite{Ishwaran:Zarepour:2002} for the Dirichlet process or \cite{Paisley:Carin:2009,Zhou:2009} for the Indian buffet process), or we can construct a slice sampler that employs a random truncation that maintains the correct posterior distribution (see \cite{Walker:2007,Ge:Chen:Wan:Ghahramani:2015} for the Dirichlet process or \cite{Teh:Gorur:Ghahramani:2007} for the Indian buffet process).

A collapsed sampler (see \cite{Ishwaran:James:2001,Neal:1998} for the Dirichlet process and \cite{Griffiths:Ghahramani:2005} for the Indian buffet process) integrates out the random measure, and works only with the cluster allocations (Dirichlet process) or latent feature allocations (Indian buffet process). Since we only observe a finite number of clusters or latent features, we do not need to introduce approximations or slice variables. We make use of the fact that the sequences obtained by integrating out the random variables are exchangeable, meaning we can adapt the predictive distributions in Equations~\ref{eqn:crp} and \ref{eqn:ibp} to give a conditional distribution $P(Z_n|Z_{-n})$. This can be combined with a likelihood term $P(X_n|Z_n, \Theta)$ to give the full conditional distribution, which can in term be used to construct a Gibbs sampler. 

%\subsection{Distributed inference methods}
\section{Distributed inference methods}
\fi 

Inference in the resulting exchangeable distributions tends to fall into two categories: uncollapsed methods that (partially, or approximately) instantiate the latent CRM or normalized CRM and alternate between sampling the latent measure and the assignments \citep{Ishwaran:Zarepour:2002,Paisley:Carin:2009,Zhou:2009,Walker:2007,Ge:Chen:Wan:Ghahramani:2015,Teh:Gorur:Ghahramani:2007}, and collapsed methods where the latent measure is integrated out \citep{Ishwaran:James:2001,Neal:1998,Griffiths:Ghahramani:2005}.  

Both approaches have their advantages and disadvantages. As discussed by \cite{Ishwaran:James:2001}, collapsed methods tend to mix slowly due to the dependency between assignments, while blocked updates mean uncollapsed methods typically have good mixing properties at convergence. However, as discussed by \cite{Neal:1998}, \sinead{Add more citations here for uncollapsed in high dimensions... Michael?}, uncollapsed methods are often slow to incorporate new components, since they typically rely on sampling unoccupied components from the prior. In high dimensions, such components are unlikely to be close to the data. Conversely, collapsed methods can make use of the data when introducing new points \cite{Neal:1998}, which tends to lead to faster convergence.

\sinead{Here mention hybrid}



A number of inference algorithms have been proposed that allow computation to be distributed across multiple machines. In an uncollapsed setting, \cite{Smyth:Welling:Asuncion:2009} proposed an approximate distributed scheme for the hierarchical Dirichlet process, which is easily adaptable to the Dirichlet process mixture model. On each local step, each node assumes that the sufficient statistics from the other nodes are unchanged from the previous global step. On global steps, the sufficient statistics are updated and new clusters are (approximately) aligned. 

As \cite{Williamson:Dubey:Xing:2013} show, this approach works well where the clusters are large, but when working with small clusters suffers from alignment issues, due to both problems matching up new clusters, and the possibility of small clusters drifting in location over the course of a local iteration.  Along a similar vein, \cite{Doshi-Velez:2009} develop a distributed inference algorithm for the IBP. Here, each processor approximates the current feature counts from the other processors with the counts from the previous time step; there is no explicit merging of new features. As we will see in Section~\ref{experiments}, this approach will lead to over-estimation of the number of new features, and poor mixing.

\cite{Williamson:Dubey:Xing:2013} proposed a distributed method based on partitioning the Dirichlet process into a mixture of conditionally independent Dirichlet processes. Inference in the conditionally independent Dirichlet process mixture models is carried out locally using a collapsed scheme. Global moves are used to move data between the conditionally independent Dirichlet processes to ensure correct mixing. While this approach works well for relatively small numbers of processors, its scalability is limited by the fact that each cluster in the overall DPMM must reside on a single processor (as discussed by \citealt{Williamson:Dubey:Xing:2013} and \citealt{Gal:Ghahramani:2014}). 

Further, the approach assumes a shared-memory architecture where there is minimal cost to moving data between processors; in a distributed-memory context this would cause significant communication bottlenecks. It also relies heavily on properties specific to the Dirichlet process; while this approach has been extended to the related Pitman-Yor process \citep{Dubey:Williamson:Xing:2014}, it is unclear how to extend to models such as the IBP.https://www.overleaf.com/project/5d72739cf71fc30001d78d63

\citet{Ge:Chen:Wan:Ghahramani:2015} propose a distributed-memory, low-communication algorithm for the Dirichlet process based on an uncollapsed approach, explicitly instantiating the cluster probabilities and parameters. A slice sampler is used to ensure only a finite number of atoms need to be represented. When new atoms are introduced by the slice sampler, a shared seed is used in the pseudo-random number generators on each node, to ensure that the same atoms are proposed without the need for direct communication. The downside of this approach is that, by necessity, the new atoms are sampled from the prior, rather than from their conditional distribution given observations. In high dimensions, this means that the proposed atoms are likely to be very far from data, and will therefore tend not to be used, resulting in slow mixing.


\sinead{There is probably more stuff since we wrote the original draft!!}
\michael{Discuss other hybrid methods}

\iffalse
A number of parallel inference algorithms have been proposed for the Dirichlet process and its variants. \cite{Smyth:Welling:Asuncion:2009} proposed an approximate distributed scheme for the hierarchical Dirichlet process, which is easily adaptable to the Dirichlet process mixture model. On each local step, each node assumes that the sufficient statistics from the other nodes are unchanged from the previous global step. On global steps, the sufficient statistics are updated and new clusters are (approximately) aligned. As \cite{Williamson:Dubey:Xing:2013} show, this approach works well where the clusters are large, but when working with small clusters suffers from alignment issues, due to both problems matching up new clusters, and the possibility of small clusters drifting in location over the course of a local iteration.

\cite{Williamson:Dubey:Xing:2013} proposed a distributed method based on partitioning the Dirichlet process into a mixture of conditionally independent Dirichlet processes. These conditionally independent Dirichlet processes are updated independently on separate processors during local steps. Global moves are used to move data between the conditionally independent Dirichlet processes to ensure correct mixing. While this approach works well for relatively small numbers of processors, its scalability is limited by the fact that each cluster in the overall DPMM must reside on a single processor (as discussed by \cite{Williamson:Dubey:Xing:2013} and \cite{Gal:Ghahramani:2014}). Further, the approach assumes a shared-memory architecture where there is minimal cost to moving data between processors; in a distributed-memory context this would cause significant communication bottlenecks.

%[Something about subcluster splits]

A more recent approach, that is explicitly designed for the distributed-memory, low-communication setting, was proposed by \cite{Ge:Chen:Wan:Ghahramani:2015}. Unlike the previously described approaches, this paper uses an uncollapsed approach, explicitly instantiating the cluster probabilities and parameters. A slice sampler is used to ensure only a finite number of atoms need to be represented. When new atoms are introduced by the slice sampler, a shared seed is used in the pseudo-random number generators on each node, to ensure that the same atoms are proposed without the need for direct communication.

The downside of this approach is that, by necessity, the new atoms are sampled from the prior, rather than from their conditional distribution given observations. In high dimensions, this means that the proposed atoms are likely to be very far from data, and will therefore tend not to be used, resulting in slow mixing.

Compared with the Dirichlet process, there has been relatively little work on distributed inference for the Indian buffet process. The main contribution in this area is by \cite{Doshi-Velez:2009}, who deploy an approach similar to that of \cite{Smyth:Welling:Asuncion:2009}. Each processor approximates the current feature counts from the other processors with the counts from the previous time step; there is no explicit merging of new features. As we will see in Section~\ref{experiments}, this approach will lead to over-estimation of the number of new features, and poor mixing.

%[sub-modular IBP??]


\fi
